Adaptive Chameleon or Stubborn Sloth: Revealing the Behavior of Large Language Models in Knowledge Conflicts

By providing external information to large language models (LLMs), tool augmentation (including retrieval augmentation) has emerged as a promising solution for addressing the limitations of LLMs' static parametric memory. However, how receptive are LLMs to such external evidence, especially when the evidence conflicts with their parametric memory? We present the first comprehensive and controlled investigation into the behavior of LLMs when encountering knowledge conflicts. We propose a systematic framework to elicit high-quality parametric memory from LLMs and construct the corresponding counter-memory, which enables us to conduct a series of controlled experiments. Our investigation reveals seemingly contradicting behaviors of LLMs. On the one hand, different from prior wisdom, we find that LLMs can be highly receptive to external evidence even when that conflicts with their parametric memory, given that the external evidence is coherent and convincing. On the other hand, LLMs also demonstrate a strong confirmation bias when the external evidence contains some information that is consistent with their parametric memory, despite being presented with conflicting evidence at the same time. These results pose important implications that are worth careful consideration for the further development and deployment of tool- and retrieval-augmented LLMs. Resources are available at https://github.com/OSU-NLP-Group/LLM-Knowledge-Conflict.

==> 080limitations.tex <==
In this study, we focus on examining the behavior of LLMs when confronted with knowledge conflicts, with the aim of informing future research and real-word applications based on retrieval- or tool-augmented LLMs. 
However, given the lack of programmatic access to LLMs currently deployed in real-world systems like New Bing, we use GPT-4 instead, with the consideration that New Bing is based on GPT-4.\footnote{\href{https://blogs.bing.com/search/march_2023/Confirmed-the-new-Bing-runs-on-OpenAI\%E2\%80\%99s-GPT-4}{https://blogs.bing.com/search/march\_2023/Confirmed-the-new-Bing-runs-on-OpenAI's-GPT-4}.}
We also experiment on ChatGPT as many plugins have been developed for it.

Another consideration is our use of prompts and instructions to steer LLMs.
While intuitively reasonable, these may not precisely align with the prompts adopted in specific applications due to their undisclosed policies.
That being said, we maintain that our current methodology does not detract from our overall findings.
